Deep Neural Compression Via Concurrent Pruning and Self-Distillation

Pruning aims to reduce the number of parameters while maintaining performance close to the original network. This work proposes a novel \emph{self-distillation} based pruning strategy, whereby the representational similarity between the pruned and unpruned versions of the same network is maximized. Unlike previous approaches that treat distillation and pruning separately, we use distillation to inform the pruning criteria, without requiring a separate student network as in knowledge distillation. We show that the proposed {\em cross-correlation objective for self-distilled pruning} implicitly encourages sparse solutions, naturally complementing magnitude-based pruning criteria. Experiments on the GLUE and XGLUE benchmarks show that self-distilled pruning increases mono- and cross-lingual language model performance. Self-distilled pruned models also outperform smaller Transformers with an equal number of parameters and are competitive against (6 times) larger distilled networks. We also observe that self-distillation (1) maximizes class separability, (2) increases the signal-to-noise ratio, and (3) converges faster after pruning steps, providing further insights into why self-distilled pruning improves generalization.

==> figures/3_monolingual_glue_ggplot.tex <==
% Textual Similarity (STS-B)
\begin{figure*}[ht]
\begin{subfigure}{.325\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{images/glue/qnli.pdf}
  \caption{Question Answering NLI (QNLI)}
  \label{fig:qnli}
\end{subfigure}%
\begin{subfigure}{.325\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{images/glue/sst-2.pdf}
  \caption{Sentiment Analysis (SST-2)}
  \label{fig:sst}
\end{subfigure}
%\hfill
%\begin{subfigure}{.249\textwidth}
%  \centering
%  \includegraphics[width=1.\linewidth]{images/glue/mnli.pdf}
%  \caption{Multi-Genre NLI (MNLI)}
%  \label{fig:mnli}
%\end{subfigure}
%
\begin{subfigure}{.325\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{images/glue/cola.pdf}
  \caption{Linguistic Acceptability (CoLA)}
  \label{fig:mnli}
\end{subfigure}
\caption{\textbf{Iterative Pruning Test Performance on GLUE tasks.}}
\label{fig:glue_pruning_methods}

\end{figure*}

==> figures/6_zero_shot_xglue_ggplot.tex <==
\begin{figure*}[ht]
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/pos.png}
  \caption{Part of Speech Tagging}
  \label{fig:pos}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/ner.png}
  \caption{Named Entity Recognition}
  \label{fig:ner}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/nc.png}
  \caption{News Classification}
  \label{fig:news}
\end{subfigure}
\hfill
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/qam.png}
  \caption{Question Answer Matching}
  \label{fig:qam}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/xnli.png}
  \caption{XNLI}
  \label{fig:xnli}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/wpr.png}
  \caption{Web-Page Ranking}
  \label{fig:wpr}
\end{subfigure}
\caption{\textbf{Zero-Shot Results After Iteratively Fine-Pruning XLM-R$_{\mathrm{Base}}$ on XGLUE tasks}.}
\label{fig:pruning_methods}
\end{figure*}

==> figures/monolingual_glue_ggplot.tex <==
\begin{figure*}[ht]
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/glue/stsb.png}
  \caption{Textual Similarity (STS-B)}
  \label{fig:sts}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/glue/sst.png}
  \caption{Sentiment Analysis (SST-2)}
  \label{fig:sst}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/glue/mrpc.png}
  \caption{Paraphrase Classif. (MRPC)}
  \label{fig:mrpc}
\end{subfigure}
\hfill
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/rte.png}
  \caption{Textual Entailment (RTE)}
  \label{fig:rte}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/mnli.png}
  \caption{Multi-Genre NLI (MNLI)}
  \label{fig:mnli}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/wnli.png}
  \caption{Reading Comprehension (WNLI)}
  \label{fig:wnli}
\end{subfigure}
\caption{\textbf{Iterative Pruning Test Performance on GLUE tasks.}}
\label{fig:pruning_methods}

\end{figure*}

==> figures/zero_shot_xglue.tex <==
\begin{figure*}[ht]
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/pos.png}
  \caption{Part of Speech Tagging}
  \label{fig:pos}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/ner.png}
  \caption{Named Entity Recognition}
  \label{fig:ner}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/nc.png}
  \caption{News Classification}
  \label{fig:news}
\end{subfigure}
\hfill
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/pawsx.png}
  \caption{Cross-lingual Adversarial Paraphrase Identification}
  \label{fig:pawsx}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/qam_pruning_results.png}
  \caption{Question Answer Matching}
  \label{fig:qam}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/qadsm_pruning_results.png}
  \caption{Question Ad Matching}
  \label{fig:qadsm}
\end{subfigure}
\hfill
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/pawsx_pruning_results.png}
  \caption{PAWS-X}
  \label{fig:pawsx_new}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/xnli_pruning_results.png}
  \caption{XNLI}
  \label{fig:xnli}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/wpr_pruning_results.png}
  \caption{Web-Page Ranking}
  \label{fig:wpr}
\end{subfigure}
\caption{Average Zero-Shot Results After Iteratively Fine-Pruning XLM-RoBERTa-Base on XGLUE tasks}
\label{fig:pruning_methods}
\end{figure*}

==> figures/zero_shot_xglue_ggplot.tex <==
\begin{figure*}[ht]
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/pos.png}
  \caption{Part of Speech Tagging}
  \label{fig:pos}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/ner.png}
  \caption{Named Entity Recognition}
  \label{fig:ner}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/nc.png}
  \caption{News Classification}
  \label{fig:news}
\end{subfigure}
\hfill
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/pawsx.png}
  \caption{Cross-lingual Adversarial Paraphrase Identification}
  \label{fig:pawsx}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/qam.png}
  \caption{Question Answer Matching}
  \label{fig:qam}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/qadsm.png}
  \caption{Question Ad Matching}
  \label{fig:qadsm}
\end{subfigure}
\hfill
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/pawsx.png}
  \caption{PAWS-X}
  \label{fig:pawsx_new}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/xnli.png}
  \caption{XNLI}
  \label{fig:xnli}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{images/xglue/ggplot/wpr.png}
  \caption{Web-Page Ranking}
  \label{fig:wpr}
\end{subfigure}
\caption{Average Zero-Shot Results After Iteratively Fine-Pruning XLM-RoBERTa-Base on XGLUE tasks}
\label{fig:pruning_methods}
\end{figure*}

==> old_method/kde_mi_estimator.tex <==
\paragraph{Mutual Information Estimation Between Pruned and Unpruned Representations}
The KDE approach of~\cite{kolchinsky2017estimating,kolchinsky2019nonlinear}; estimates the mutual information between the input and the hidden layer activity by assuming that the hidden activity is distributed as a mixture of Gaussians. This assumption is well-suited to the present setting under the following interpretation: we take the input activity to be distributed as delta functions at each example in the dataset, corresponding to a uniform distribution over these specific samples. In other words, we assume that the empirical distribution of input samples is the true distribution. Next, the hidden layer activity h is a deterministic function of the input. As mentioned in the main text and discussed in more detail in Appendix C, without the assumption of noise, this would have infinite mutual information with the input. We therefore assume for the purposes of analysis that Gaussian noise of variance $\sigma^2$ is added, that is, $T = h + \epsilon$ where $\epsilon \sim \mathcal{N}(0, \sigma^2 I)$. Under these assumptions, the distribution of $T$ is genuinely a mixture of Gaussians, with a Gaussian centered on the hidden activity corresponding to each input sample. We emphasize again that the noise $\epsilon$ is added solely for the purposes of analysis, and is not present during training or testing the network. In this setting, an upper bound for the mutual information with the input is ~\cite{kolchinsky2017estimating,kolchinsky2019nonlinear}.

\begin{equation}
I(T; X) \leq -\frac{1}{P}\sum_i \log \frac{1}{P} \sum_j \exp\Big( -\frac{1}{2} \frac{||\vec{z}_i - \vec{z}_j ||^2_2}{\sigma^2}\Big)
\end{equation}

where $P$ is the number of training samples and hi denotes the hidden activity vector in response to input sample $i$. Similarly, the mutual information with respect to the output can be calculated as

\begin{equation}
\begin{gathered}
I(T; Y ) = H(T) - H(T|Y)   
\leq -\frac{1}{P}\sum_i \log \frac{1}{P} \sum_j \exp\Big( -\frac{1}{2} \frac{||\vec{z}_i - \vec{z}_j ||^2_2}{\sigma^2}\Big) \\
- \sum_{l}^{L}p_l \Bigg[\frac{1}{P_l}\sum_{i, Y_i=l} \log \frac{1}{P_l} \sum_{j, Y_j=l} \exp\Big( -\frac{1}{2} \frac{||\vec{z}_i - \vec{z}_j ||^2_2}{\sigma^2}\Big)\Bigg]
\end{gathered}
\end{equation}

where $L$ is the number of output labels, $P_l$ denotes the number of data samples with output label $l, p_l = P_l/P$ denotes the probability of output label $l$, and the sums over $i, Y_i = l$ indicate a sum over all examples with output label $l$.

==> old_method/mi.tex <==
From a perspective of information theory, knowledge transfer can be expressed as retaining high mutual information between the layers of the teacher and the student networks. More specifically, consider an input random variable x drawn from the target data distribution $p(x)$ and $K$ pairs of layers $R = \{(T(k), S(k))\}^K_{k=1}$, where each pair $(T(k), S(k))$ is selected from the teacher network and the student network respectively. Feedforwarding the input $x$ through the networks induces K pairs of random variables $\{(t(k), s(k))\}^K_{k=1}$ which indicate activations of the selected layers, e.g., $t(k) = T(k)(x)$. The mutual information between the pair of random variables (t, s) is defined by:
\beg0in{equation}
I(t; s) = H(t) - H(t|s) = - \mathbb{E}_t[\log p(t)] + \mathbb{E}_{t,s}[\log p(t|s)]    
\end{equation}
where the entropy $H(t)$ and the conditional entropy $H(t|s)$ are derived from the joint distribution $p(t, s)$. Empirically, the joint distribution $p(t, s)$ is a result of aggregation over the layers with input $x$ sampled from the input distribution

==> old_method/sdp_smoothens.tex <==
\subsection{Self-Distillation Smoothens The Loss Surface}
Before understanding how self-distillation improves model compression, we first need to understand how self-distillation improves generalization without any compression. To this end, we quantify smoothness of the loss surface and how this correlates to the generalization properties of self-distilled models. Intuitively, we would expect that networks with generalizable representations would consist of relatively small weight norms. Hence, we may infer that self-distilled models may have a weight regularization effect which in turn complements magnitude-based pruning as it becomes easier to select weights with lower magnitudes. Another explanation of why distillation improves generalization is that the teacher network logits provide more semantic information about class similarities which leads better estimates of the true class boundaries. 

==> related_work/kd.tex <==
% USE BELOW TO FINISH. 

Various extensions of this approach have been recently proposed, where instead of output predictions, the student tries to match other statistics from the teacher model such as intermediate feature representations~\cite{romero2014fitnets}, Jacobian matrices~\cite{srinivas2018knowledge}, distributions ~\cite{huang2017like}, Gram matrices~\cite{yim2017gift}. Additional developments on knowledge distillation include its extensions to Bayesian settings~\cite{korattikara2015bayesian,vadera2020generalized}, uncertainty preservation~\cite{tran2020hydra}, reinforcement learning~\cite{hong2019collaborative,teh2017distral,ghosh2017divide}, online distillation~\cite{lan2018knowledge}, zero-shot learning~\cite{nayak2019zero},
multi-step knowledge distillation~\cite{mirzadeh2020improved}, tackling catastrophic forgetting~\cite{mirzadeh2020improved}, transfer of relational knowledge~\cite{park2019relational}, adversarial distillation~\cite{wang2018kdgan}. Recently~\cite{phuong2019towards} analyzed why the student model is able to mimic teacher model
in knowledge distillation and ~\citeauthor{menon2020distillation} presented a statistical perspective on distillation.

==> related_work/label_smoothing.tex <==
\paragraph{Label Smoothing}
To identify whether the generalization benefits are specific to the logits learned from a fine-tuned network, we can also analyse whether label smoothing of targets has a similar generalization effect. If so, this implies soft targets, regardless if they are learned or not, lead to better generalization. Mueller et al.~\cite{muller2019does} have already found that while label smoothing improves generalization via improved model calibration in standard supervised learning, in the KD setup, learning from a teacher network that is trained with label smoothing \emph{reduces} performance of the student network. They find that label smoothing leads to tight clustering of representations from the same class which corresponds to information loss in the logits w.r.t similarities between instances of different class, which is useful for distillation. In other words, because the intra-class distances between instances of different classes is larger in networks trained using label smoothing, it provides less information about the class boundaries in the logits which distilled networks greatly benefit from. This justifies, why these distilled logits may be useful for our proposed SDP. 

% Label smoothing prevents the network from becoming over-confident, improves generalization by better model calibration and encourages the representations of training examples from the same class to group in tight clusters. This results in loss of information in the logits about resemblances between instances of different classes, which is necessary for distillation, but does not hurt generalization or calibration of the model’s predictions.

% For a teacher trained with hard targets ($\alpha$ = 0.0), we observe that examples are distributed in broad clusters, which means that different examples from the same class can have very different similarities to other classes. For a teacher trained with label smoothing, we observe the opposite behavior. Label smoothing encourages examples to lie in tight equally separated clusters, so every example of one class has very similar proximities to examples of the other classes. Therefore, a teacher with better test accuracy is not necessarily the one that distills better

==> sup/probabilistic_mi.tex <==
Our goal now is to estimate the MI $I(Z^T; Z^S)$ as $I(Z^T; Z^S) = \int \int p_{Z^T, Z^S}(z^T, z^S)\log p_{Z^T Z^S}(z^T, z^S) p_{Z^T}(z^T) p_{z^S}(y)dz^Tdz^S$, where $p_{Z^T Z^S}(z^T, z^S)$ is the joint density of $Z^T$ and $Z^S$ and $p_{Z^S}(z^{S}) = RY p_{XY}(x, y)dy$ and $p_Y(y) = RX p_{XY}(x, y)dx$ are the marginal densities. These theoretical quantities are not available to us and we must somehow estimate $\hat{I}(X; Y)$ directly from the representations. To estimate MI between continuous random variables given the test set batch representations, we use a k-NN based histogram binning which partitions the supports $\mathcal{Z}^S , \mathcal{Z}^T$ into a finite number of bins of equal or unequal (adaptive) size and estimates $\hat{I}(X; Y)$ based on discrete counts in each bin. We then formulate the MI as \autoref{eq:mi},

==> sup/snr_additional.tex <==
% This is often explicitly achieved in deep metric learning objectives using margin-based losses and contrastive losses maximize the similarity of positive pairs and minimize the similarity of negative pairs. Here, we posit that relative similarities between representations are encoded in the soft labels given by the teachers, producing similar dynamics to metric learned models. Moreover, they force the representations to have small intra-class distances and large inter-class distance. 

% Margin-based machine learning models maximize the boundary between classes during optimization, aiming to find a classification boundary that generalizes well on the test set. Intuitively, we expect SDP to implicitly force better separation between classes as we know from previous work \textbf{cite here} which finds self-distillation to do so. From this we can define a general scheme that measures the signal-to-noise ratio in $f^S$ as the means to understand how SDP may generalize better than magnitude-based pruning without self-distillation. 

%Let us define the SNR as $1/NC\sum_{i}^{N}\sum_{c=1}^{C}\frac{\mathbb{F}(\mat{Z}_c, \mathrm{shuffle}(\mat{Z}_c))}{\mathbb{F}}$
